Out-of-distributional risk bounds for neural operators with applications to the Helmholtz equation

Despite their remarkable success in approximating a wide range of operators defined by PDEs, existing neural operators (NOs) do not necessarily perform well for all physics problems. We focus here on high-frequency waves to highlight possible shortcomings. To resolve these, we propose a subfamily of NOs enabling an enhanced empirical approximation of the nonlinear operator mapping wave speed to solution, or boundary values for the Helmholtz equation on a bounded domain. The latter operator is commonly referred to as the ''forward'' operator in the study of inverse problems. Our methodology draws inspiration from transformers and techniques such as stochastic depth. Our experiments reveal certain surprises in the generalization and the relevance of introducing stochastic depth. Our NOs show superior performance as compared with standard NOs, not only for testing within the training distribution but also for out-of-distribution scenarios. To delve into this observation, we offer an in-depth analysis of the Rademacher complexity associated with our modified models and prove an upper bound tied to their stochastic depth that existing NOs do not satisfy. Furthermore, we obtain a novel out-of-distribution risk bound tailored to Gaussian measures on Banach spaces, again relating stochastic depth with the bound. We conclude by proposing a hypernetwork version of the subfamily of NOs as a surrogate model for the mentioned forward operator.

==> Generalization_error_bound/6.tex <==


In this last section, we prove Theorem~\ref{Rademacher for standard NO} (Rademacher Complexity for NOs).
The idea behind the proof is as follows. 
The Rademacher Complexity, $\mathfrak{R}^n_{\mathrm{S}}(\mathscr{F}_{\no})$, is evaluated by using \emph{Dudley’s Theorem} (\cref{Dudley Theorem}, and \citet{Kakade, bartlett2017spectrally}).
The upper bound is then determined by the \emph{covering number} (as defined in \cref{Covering Number}). Since NOs are parameterized by their weight matrices and (kernel) Lipschitz continuous functions, the evaluation of the covering number ultimately involves analyzing these components, by using \citet{wainwright} and \citet{gottlieb2016adaptive}, respectively. 
Theorem~\ref{Rademacher for multiplicative NO} (Rademacher Complexity of the proposed network(s)) can also be proven by the same argument.
For details of the proof, see Appendix~\ref{Appendix3}.

\begin{proof}
%[Proof of Theorem~\ref{Rademacher for standard NO}]
By employing Lemma A.5 in \citet{bartlett2017spectrally} or Theorem 1.1 in \citet{Kakade}, we have
\begin{equation}
\mathfrak{R}^n_{\mathrm{S}}(\mathscr{F}_{\no}) \leq \inf_{\alpha \geq 0} \left\{ 4\alpha + \frac{12}{\sqrt{n}}\int_{\alpha}^{\infty}\left(\log N(\varepsilon, \mathscr{F}_{\no}, \left\| \cdot \right\|_{\mathrm{S}} )  \right)^{\frac{1}{2}} d\varepsilon \right\}
\label{Rademacher Complexity-covering number}
\end{equation}
where $\left\| f \right\|_{\mathrm{S}}:= \left(\frac{1}{n}\sum_{i=1}^{n}f(a_i, u_i)^2 \right)^{\frac{1}{2}}$.
Here, we denote by $N(\varepsilon, \mathscr{F}, \|\cdot\|)$ the covering number of the function space $\mathscr{F}$ which means 
the minimal cardinality of a subset $C \subset \mathscr{F}$ that covers $\mathscr{F}$ at scale $\varepsilon$ with respect to the norm $\|\cdot\|$. 
In the following, we will estimate the covering number $N(\varepsilon, \mathscr{F}_{\no}, \left\| \cdot \right\|_{\mathrm{S}} )$.
\par
Let $f=\ell(\Gcal(\cdot), \cdot)$ and $f^{\prime}=\ell(\Gcal^{\prime}(\cdot), \cdot)$ where $\Gcal, \Gcal^{\prime} \in \no$.
By (i) of Assumption \ref{Assumption1}, we calculate 
\begin{equation}
\left|f(a,u)-f^{\prime}(a,u)\right| 
= \left|\ell(\Gcal(a),u)- \ell(\Gcal^{\prime}(a),u)\right|
\leq \rho \left\| \Gcal(a) -\Gcal^{\prime}(a) \right\|_{\Lp(D;\mathbb{R}^{d_u})}. \label{covering number-estimation 1}
\end{equation}
Denoting by
\[
\Gcal_{\ell}:=(W_{\ell}+\bk_{\ell})\circ \sigma (W_{\ell-1}+\bk_{\ell-1})\circ \cdots \circ \sigma (W_{0}+\bk_{0}),
\]
\[
\Gcal^{\prime}_{\ell}:=(W^{\prime}_{\ell}+\bk^{\prime}_{\ell})\circ \sigma (W^{\prime}_{\ell-1}+\bk^{\prime}_{\ell-1})\circ \cdots \circ \sigma (W^{\prime}_{0}+\bk^{\prime}_{0}),
\]
the quantity $\left\| \Gcal(a) -\Gcal^{\prime}(a) \right\|_{\Lp(D;\mathbb{R}^{d_u})}$ is evaluated by
\begin{equation}
\begin{split}
&
\left\| \Gcal(a) -\Gcal^{\prime}(a) \right\|_{\Lp(D;\mathbb{R}^{d_u})} = \left\| \Gcal_{L}(a) -\Gcal^{\prime}_{L}(a) \right\|_{\Lp(D;\mathbb{R}^{d_{L+1}})}
\\
&
= \Bigl\|(W_{L}+\bk_{L})\circ \sigma( \Gcal_{L-1}(a)) - (W_{L}+\bk_{L})\circ \sigma( \Gcal_{L-1}^{\prime}(a))
\\
& \hspace{2cm}
+(W_{L}+\bk_{L})\circ \sigma(\Gcal_{L-1}^{\prime}(a)) - (W^{\prime}_{L}+\bk^{\prime}_{L})\circ  \sigma(\Gcal_{L-1}^{\prime}(a)) \Bigr\|_{\Lp(D;\mathbb{R}^{d_{L+1}})}
\\
&
\underset{Assumption\ref{Assumption2}(vi)}{}
\\
&
\leq 
\Biggl(
\underbracket{\left\| W_{L} \right\|_{\mathrm{op}}}_{\underset{(\ref{covering number-estimation 3})}{\leq} C_w}
+ 
\underbracket{\left\| \bk_{L} \right\|_{\mathrm{op}}}_{\underset{(\ref{covering number-estimation 4})}{\leq} C_k}
\Biggr) C_{\sigma} \left\|\Gcal_{L-1}(a)-\Gcal^{\prime}_{L-1}(a)\right\|_{\Lp(D;\mathbb{R}^{d_L})}
\\
& \hspace{2cm}
+\left(\left\| W_{L}-W^{\prime}_{L} \right\|_{\mathrm{op}}
+ \left\| \bk_{L}-\bk^{\prime}_{L} \right\|_{\mathrm{op}} \right) C_{\sigma}
\left\|\Gcal^{\prime}_{L-1}(a)\right\|_{\Lp(D;\mathbb{R}^{d_L})},
\end{split}
\label{covering number-estimation 2}
\end{equation}
where $\left\|\cdot \right\|_{\mathrm{op}}$ is the Operator norm.
Here, we have employed the following estimations:
\begin{equation}
\left\| W_{L}g \right\|^{2}_{\Lp(D;\mathbb{R}^{d_{L+1}})}\leq 
\int_{D}
\underbracket{
\left\|W_{L}g(x) \right\|^{2}_{2}
}_{\leq \left\|W_{L}\right\|^{2}_{\mathrm{F}}\left\|g(x)\right\|^{2}_{2}}
dx 
\underset{\text{Assumption} \ref{Assumption2}(i)}{\leq} C^{2}_{w}
\left\|g \right\|^{2}_{\Lp(D;\mathbb{R}^{d_{L}})},
\label{covering number-estimation 3}
\end{equation}
\begin{equation}
\begin{split}
\left\| \bk_{L}g \right\|^{2}_{\Lp(D;\mathbb{R}^{d_{L+1}})}
\leq 
\int_{D} 
\underbracket{\left\|\int_{D}
\bk_{L}(x,y)g(y)dy \right\|^{2}_{2}
}_{\leq \left(\sum_{i,j}
\left\|k_{L,ij}(x,\cdot)\right\|^{2}_{\Lp(D)} \right) \left\|g\right\|^{2}_{\Lp(D;\mathbb{R}^{d_{L}}}}
dx 
& \leq \left\|\bk_{L}\right\|_{\Lp, \mathrm{F}}^{2}
\left\|g \right\|^{2}_{\Lp(D;\mathbb{R}^{d_{L}})}
\\
&\hspace{-1cm}
\underset{\text{Assumption} \ref{Assumption2}(ii)}{\leq}
C^{2}_{k}\left\|g \right\|^{2}_{\Lp(D;\mathbb{R}^{d_{L}})},
\label{covering number-estimation 4}
\end{split}
\end{equation}
for $g \in \Lp(D; \mathbb{R}^{d_L})$,
where $\left\| \cdot \right\|_{2}$ is the $\ell_2$-norm.
By the same argument in (\ref{covering number-estimation 2})--(\ref{covering number-estimation 4}), we evaluate
\begin{equation}
\begin{split}
& \left\|\Gcal_{L-1}(a)-\Gcal^{\prime}_{L-1}(a)\right\|_{\Lp(D;\mathbb{R}^{d_L})}
\\
&
\leq (C_w +C_k)C_{\sigma}\left\|\Gcal_{L-2}(a)-\Gcal^{\prime}_{L-2}(a)\right\|_{\Lp(D;\mathbb{R}^{d_{L-1}})}
\\
& \hspace{0cm}
+\left(\left\| W_{L-1}-W^{\prime}_{L-1} \right\|_{\mathrm{op}}
+ \left\| \bk_{L-1}-\bk^{\prime}_{L-1} \right\|_{\mathrm{op}} \right) C_{\sigma}
\left\|\Gcal^{\prime}_{L-2}(a)\right\|_{\Lp(D;\mathbb{R}^{d_{L-1}})}.
\end{split}
\label{covering number-estimation 5}
\end{equation}
By repeatedly evaluating $\left\|\Gcal_{\ell}(a)-\Gcal^{\prime}_{\ell}(a)\right\|_{\Lp(D;\mathbb{R}^{d_{\ell+1}})}$ ($\ell=L,L-1,...,0$), we obtain 
\begin{equation}
\begin{split}
& \left\|\Gcal(a)-\Gcal^{\prime}(a)\right\|_{\Lp(D;\mathbb{R}^{d_u})}
\\
&
\leq \left\{(C_w +C_k)C_{\sigma}\right\}^{L}
\underbracket{
\left\|(W_0 + \bk_0)(a)-(W^{\prime}_0 + \bk^{\prime}_0)(a)\right\|_{\Lp(D;\mathbb{R}^{d_{1}})}}
_{
\underset{\text{Assumption} \ref{Assumption2}(iii)}{}\leq C_a (\left\| W_{0}-W^{\prime}_{0} \right\|_{\mathrm{op}}
+ \left\| \bk_{0}-\bk^{\prime}_{0} \right\|_{\mathrm{op}})}
\\
& \hspace{0cm}
+\sum_{\ell=0}^{L-1}\left(\left\| W_{\ell+1}-W^{\prime}_{\ell+1} \right\|_{\mathrm{op}}
+ \left\| \bk_{\ell+1}-\bk^{\prime}_{\ell+1} \right\|_{\mathrm{op}} \right) 
\\
&\hspace{3cm}
\times \underbracket{(C_w + C_k)^{L-1-\ell} C^{L-\ell}_{\sigma}
\left\|\Gcal^{\prime}_{\ell}(a)\right\|_{\Lp(D;\mathbb{R}^{d_{\ell+1}})}}
_{\underset{(\ref{covering number-estimation 7})}{}\leq \left\{(C_w +C_k)C_{\sigma}\right\}^{L}C_a \ }
\\
&
\leq \left\{(C_w+C_k)C_{\sigma}\right\}^{L}C_a \sum_{\ell=0}^{L}\left(\left\| W_{\ell}-W^{\prime}_{\ell} \right\|_{\mathrm{op}}
+ \left\| \bk_{\ell}-\bk^{\prime}_{\ell} \right\|_{\mathrm{op}} \right).
\end{split}
\label{covering number-estimation 6}
\end{equation}
Here, we have employed the following estimation:
\begin{equation}
\left\| \Gcal^{\prime}_{\ell} \right\|^{2}_{\Lp(D;\mathbb{R}^{d_{\ell+1}})}
\leq 
(C_w+C_k)^{\ell+1}C_{\sigma}^{\ell}C_a.
\label{covering number-estimation 7}
\end{equation}
Furthermore, by using ideas of (\ref{covering number-estimation 3}) and (\ref{covering number-estimation 4}), we estimate 
\begin{equation}
\begin{split}
\left\| W_{\ell}-W^{\prime}_{\ell} \right\|_{\mathrm{op}} & \leq \left\| W_{\ell}-W^{\prime}_{\ell} \right\|_{\mathrm{F}}
\\
&
\leq
\sum_{j=1}^{d_{\ell+1}}\sum_{i=1}^{d_{\ell}} |w_{\ell, ij}-w^{\prime}_{\ell, ij}|
\leq
\sum_{j=1}^{d_{\ell+1}}\sum_{i=1}^{d_{\ell}}C_w \left|\frac{w_{\ell, ij}}{C_w}-\frac{w^{\prime}_{\ell, ij}}{C_w}\right|,
\end{split}
\label{covering number-estimation 8}
\end{equation}
\begin{equation}
\begin{split}
&
\left\| \bk_{\ell}-\bk^{\prime}_{\ell} \right\|_{\mathrm{op}} 
%\leq
%|D|
%\left\| k_{\ell}-k^{\prime}_{\ell} \right\|_{\mathrm{F}, \infty}
%\\
%&
\leq
\sum_{j=1}^{d_{\ell+1}}\sum_{i=1}^{d_{\ell}}
|D| \left\|k_{\ell, ij}-k^{\prime}_{\ell, ij}\right\|_{\boldsymbol{\mathrm{L}}^{\infty}(D\times D;\mathbb{R})}
\leq
\sum_{j=1}^{d_{\ell+1}}\sum_{i=1}^{d_{\ell}} |D| C_{\alpha} \left\|\frac{k_{\ell, ij}}{C_{\alpha}}-\frac{k^{\prime}_{\ell, ij}}{C_{\alpha}}\right\|_{\boldsymbol{\mathrm{L}}^{\infty}(D\times D;\mathbb{R})}.
\end{split}
\label{covering number-estimation 9}
\end{equation}
Combining (\ref{covering number-estimation 1}), (\ref{covering number-estimation 6}), (\ref{covering number-estimation 8}), and (\ref{covering number-estimation 9}), the norm $\left\|f -f^{\prime} \right\|_{\mathrm{S}}$ is estimated by
\[
\begin{split}
&\left\|f -f^{\prime}\right\|_{\mathrm{S}}
=
\left(\frac{1}{n}\sum_{i=1}^{n}|f(a_i,u_i) -f^{\prime}(a_i,u_i)|^2 \right)^{\frac{1}{2}}
\\
&
\leq
\sum_{\ell=0}^{L}
\sum_{j=1}^{d_{\ell+1}}
\sum_{i=1}^{d_{\ell}}
\Biggl[
\rho
\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a C_w 
\left|\frac{w_{\ell, ij}}{C_w}-\frac{w^{\prime}_{\ell, ij}}{C_w}\right|
\\
&
\hspace{3cm}
+
\rho
\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a |D| C_{\alpha} 
\left\|\frac{k_{\ell, ij}}{C_{\alpha}}-\frac{k^{\prime}_{\ell, ij}}{C_{\alpha}}\right\|_{\boldsymbol{\mathrm{L}}^{\infty}(D\times D;\mathbb{R})}
\Biggr],
\end{split}
\]
which implies that we have
\begin{equation}
\begin{split}
&N(\varepsilon, \mathscr{F}_{\no}, \left\| \cdot \right\|_{\mathrm{S}} )
\\
&
\leq 
\prod_{\ell=0}^{L}\prod_{j=1}^{d_{\ell+1}}
\prod_{i=1}^{d_{\ell}}
N\left(\frac{\varepsilon}
{2\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a C_w}, [-1,1], |\cdot|
\right)
\\
&
\times
N\left(\frac{\varepsilon}
{2\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a |D| C_{\alpha}}, \mathcal{F}_{C_{\beta}}, \left\|\cdot\right\|_{\boldsymbol{\mathrm{L}}^{\infty}(D\times D; \mathbb{R})}
\right),
\end{split}
\label{covering number-estimation 10}
\end{equation}
where $\mathcal{F}_{C_{\beta}}:=\{k:D \times D \to [-1,1]\ |\ k\ \text{is}\ C_{\beta}-Lipschitz \}$ (see (vi) in Assumption \ref{Assumption2}).
\par
By taking logarithmic functions in (\ref{covering number-estimation 10}), we have 
\begin{equation}
\begin{split}
&\log N(\varepsilon, \mathscr{F}_{\no}, \left\| \cdot \right\|_{\mathrm{S}} )
\\
&
\leq 
\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\Biggl\{
\underbracket{
\log
N\left(\frac{\varepsilon}
{2\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a C_w}, [-1,1], |\cdot|
\right)
}_{=:H_w(\varepsilon)}
\\
&\hspace{1cm}
+
\underbracket{
\log
N\left(\frac{\varepsilon}
{2\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a |D| C_{\alpha}}, \mathcal{F}_{C_{\beta}}, \left\|\cdot\right\|_{\boldsymbol{\mathrm{L}}^{\infty}(D\times D; \mathbb{R})}
\right)}_{=:H_k(\varepsilon)}
\Biggr\}.
\end{split}
\label{log-covering}
\end{equation}
By using Example 5.3 of \citet{wainwright} and Lemma 4.2 of \citet{gottlieb2016adaptive}, we estimate $H_w$ and $H_k$, respectively as follows:
\begin{equation}
\begin{split}
H_w(\varepsilon) & \leq 
\log \left(1+ \frac{2\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a C_w}{\varepsilon}\right)
\\
&
\leq
\left( \frac{I_w}{\varepsilon} \right) \leq
\left( \frac{I_w}{\varepsilon} \right)^{\hat{d}+1}, \ \ \mbox{for} \ 0< \varepsilon < 2\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a C_w,
\end{split}
\label{estimation H_w}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{split}
& H_k(\varepsilon) \leq 
\left(\frac{
8C_{\beta}\mathrm{diag}(D \times D)
\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a |D| C_{\alpha}
}{\varepsilon} \right)^{\hat{d}}
\\
&
\times
\log \left(\frac{
16 \left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a |D| C_{\alpha}
}{\varepsilon}\right)
\\
&
\leq
\left(\frac{I_k}{\varepsilon} \right)^{\hat{d}+1},
\ \ \mbox{for} \ 0 < \varepsilon < 2\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a |D| C_{\alpha},
\end{split}
\label{estimation H_k}
\end{equation}
where we denoted by
\[
I_w:=2\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a C_w,
\]
\[
I_k:=8\max\left\{C_{\beta}\mathrm{diag}(D\times D), 2 \right\}\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a |D| C_{\alpha}.
\]
By employing (\ref{log-covering}), (\ref{estimation H_w}), and (\ref{estimation H_k}), we calculate
\[
\int_{\alpha}^{\infty}\left(\log N(\varepsilon, \mathscr{F}_{\no}, \left\| \cdot \right\|_{\mathrm{S}} )  \right)^{\frac{1}{2}} d\varepsilon
\leq
\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)^{\frac{1}{2}}
\underbracket{
\int_{\alpha}^{\infty}(H_w(\varepsilon)+H_k(\varepsilon))^{\frac{1}{2}}d\varepsilon
}
_{=:(\ast)}
\]
\[
\begin{split}
& (\ast) \leq
\int_{\alpha}^{\infty}
H_w(\varepsilon)^{\frac{1}{2}} d\varepsilon
+
\int_{\alpha}^{\infty}
H_w(\varepsilon)^{\frac{1}{2}} d\varepsilon
\\
&
\leq
\int_{\alpha}^{2\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a C_w}\left( \frac{I_w}{\varepsilon} \right)^{\frac{\hat{d}+1}{2}}d\varepsilon
\\
& \hspace{3cm}
+\int_{\alpha}^{2\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a |D| C_{\alpha}}\left( \frac{I_k}{\varepsilon} \right)^{\frac{\hat{d}+1}{2}}d\varepsilon
\\
&
\leq
\left(I_{w}^{\frac{\hat{d}+1}{2}}
+
I_{k}^{\frac{\hat{d}+1}{2}}
\right)
\frac{2}{\hat{d}-1}\alpha^{-\frac{\hat{d}-1}{2}} 
\\
&
\leq
\frac{4}{\hat{d}-1}
\left(
\max\left[2C_w, 8|D| C_{\alpha}\max\left\{C_{\beta} \mathrm{diag}(D\times D), 2\right\} \right]\left( \sum_{\ell=0}^{L}d_{\ell}d_{\ell+1} \right)
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a
\right)^{\frac{\hat{d}+1}{2}}
\alpha^{-\frac{\hat{d}-1}{2}},
\end{split}
\]
that is, we have by (i) of Assumption \ref{Assumption2}.
\[
\begin{split}
&
\int_{\alpha}^{\infty}\left(\log N(\varepsilon, \mathscr{F}_{\no}, \left\| \cdot \right\|_{\mathrm{S}} )  \right)^{\frac{1}{2}} d\varepsilon
\\
&
\leq
\underbracket{
\frac{4}{\hat{d}-1}
\left(
\max\left[2C_w, 8|D| C_{\alpha}\max\left\{C_{\beta} \mathrm{diag}(D\times D), 2\right\} \right]
(LC_{d}^{2})^{\frac{\hat{d}+2}{\hat{d}+1}}
\rho\left\{(C_w+C_k)C_{\sigma}
\right\}^{L}C_a
\right)^{\frac{\hat{d}+1}{2}}
}
_{=:K} \ 
\alpha^{-\frac{\hat{d}-1}{2}}
\end{split}
\]
which implies that we conclude that with (\ref{Rademacher Complexity-covering number})
\[
\begin{split}
&
\mathfrak{R}^n_{\mathrm{S}}(\mathscr{F}_{\no}) \leq 4 \inf_{\alpha \geq 0} \left\{ \alpha
+
\underbracket{
\frac{3K}{\sqrt{n}}
}_{=:K^{\prime}}
\alpha^{-\frac{\hat{d}-1}{2}}\right\}
\\
&
=
4\left( \left(\frac{(\hat{d}-1)K^{\prime}}{2} \right)^{\frac{2}{\hat{d}+1}} 
+
K^{\prime}
\left(\frac{(\hat{d}-1)K^{\prime}}{2} \right)^{\frac{2}{\hat{d}+1} \left(-\frac{\hat{d}-1}{2}\right)}
\right)
=\gamma L^{\frac{\hat{d}+2}{\hat{d}+1}} \left\{(C_w+C_k)C_{\sigma}
\right\}^{L}\left(\frac{1}{n}\right)^{\frac{1}{\hat{d}+1}}
\end{split}
\]
where $\gamma$ is the positive constant defined by
\begin{equation}
\begin{split}
\gamma
&
:=4
\left\{
\left(\frac{\hat{d}-1}{2} \right)^{\frac{2}{\hat{d}+1}}
+
\left(\frac{\hat{d}-1}{2} \right)^{-\frac{\hat{d}-1}{\hat{d}+1}}
\right\}
\left(\frac{12}{\hat{d}-1} \right)^{\frac{2}{\hat{d}+1}}
\\
& \hspace{3cm}
\times
\max\left[2C_w, 8|D| C_{\alpha}\max\left\{C_{\beta} \mathrm{diag}(D\times D), 2\right\} \right]
C_{d}^{\frac{2(\hat{d}+2)}{\hat{d}+1}}
\rho C_a.
\label{definition of gamma}
\end{split}
\end{equation}
\end{proof}


==> JCP-experiments/1.tex <==
% ---------------------------
\section{Neural network reconstruction of the wavefield at $15$ Hz.} \label{Appendux:15Hz_experiment}
To complement we show the results for three realization of wave speeds in the context of 
Experiment described in the main part of the paper for frequency $\omega/(2\pi)$ set
15 \si{\Hz}.


% ---------------------------
\setlength{\modelwidth} {4cm}
\setlength{\modelheight}{4cm}
\graphicspath{{Figures/results_experiment2_15Hz/}}
% ---------------------------
\begin{figure}[ht!]\centering
\input{Figures/results_experiment2_15Hz/skeleton_oneline_model2b} 
\vspace*{2em}

\input{Figures/results_experiment2_15Hz/skeleton_oneline_model1b}

    \caption{\small{ 
            %\textbf{(Real part) of the pressure field reconstructed by
             Pressure field (15 \si{\Hz}) reconstructed for 
             Experiment 2 (\cref{experiment2,figure:cp-GRF:experiment2}) 
             at frequency \num{15} \si{\Hz}
             with the different architectures for two GRF 
             realizations of the wave speed. 
             \textit{Left column} shows independent GRF realization of the wave
             speed (see \cref{eq:Helmholtz}).  
             \textit{Second column} shows the real and imaginary parts
             of the pressure field solution to the wave PDE at frequency
             15 \si{\Hz}, 
             obtained with software \texttt{hawen} \citep{faucher2021hawen}, 
             which we consider as the \emph{reference solution},
             see \cref{eq:Helmholtz}. 
             \textit{Other columns} show the approximated reconstructions 
             using the different architectures:
             \textit{FNO}, see \citet{kovachki2021neural}; 
             $\multiplicative$ structure ($\MFNO$, see~\cref{MNO}); 
             and the solutions provided by $\FNONeXt$, \cref{FNO+epsilon}.
             In each case, we show the real and imaginary 
             parts of the pressure fields, and 
             the relative error with the reference 
             solution on a logarithmic scale.
             }}


\label{figure:results-experiment2_15Hz}
\end{figure}
We see that the best reconstructions are obtained using 
architecture ($\FNONeXt$)v2, which is expected as
it uses multiple layers. The reconstruction with FNO is less accurate than the others, 
and we observe that ($\FNONeXt$)v1 is slightly more 
accurate than the architecture $\MNO$ in all cases.

==> JCP-experiments/2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Out-of-distribution}\label{Out-of-distribution}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We present some of the wave field reconstruction of the network on each experiment. See refer the reader to \cref{table:ood} for the values. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%OOD1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{OOD 1}
We chose $3$ realizations of all the previously trained NNs, with the dataset at $15$ Hz, and the parameters  $\boldsymbol{\lambda} = (1, 1)$, wavespeed range of $[1500,5000]$, and we tested in another GRF. In this set family, we keep the isotropic behaviour of the original data, however we move the value to ${\boldsymbol{\lambda}}_{\mathrm{OOD1}} = (0.20, 0.20)$. The range is kept in  $[1500,5000]$. The visualization of three random realizations of $c$ are presented in \cref{OOD:set1} for $15$Hz and only the real part of the field, the imaginary part is also recovered but not shown.

\setlength{\modelwidth} {4cm}
\setlength{\modelheight}{4cm}

\begin{figure}[ht!]\centering
\input{Figures/OOD_main_paper/set0/skeleton_online_set0_appendix} 
    \caption{\small{ 
            %\textbf{(Real part) of the pressure field reconstructed by
             Pressure field reconstructed for 
             Experiment 2 (\cref{experiment2,figure:cp-GRF:experiment2}) 
             at frequency \num{15} \si{\Hz} trained with \emph{isotropic Whittle–Mat\'ern covariance} 
             $\boldsymbol{\lambda} = (1, 1)$, and wavespeed range of $(1500,5000)$ \cref{eq:lambda_cov} and from \cref{table:ood}
             ${\boldsymbol{\lambda}}_{\mathrm{OOD1}} = (0.20, 0.20)$, and wavespeed range of $(1500,5000)$
             with the different architectures for multiple realizations of the new GRF
             \emph{out-of distribution},
             realizations of the wave speed. 
             \textit{Left column} shows independent GRF realization of the wave
             speed (see \cref{Euler_equation}).  
             \textit{Second column} shows the real part % and imaginary part
             of the pressure field solution to the wave PDE at frequency
             15 \si{\Hz}, 
             obtained with software \texttt{hawen} \citep{faucher2021hawen}, 
             which we consider as the \emph{reference solution},
             see \cref{Euler_equation}. 
             \textit{Other columns} show the approximated reconstructions 
             using the different architectures:
             \textit{FNO}, see \citet{kovachki2021neural}; 
             $\multiplicative$ structure ($\MFNO$, see~\cref{MNO}); 
             and the solutions provided by $\FNONeXt$, \cref{FNO+epsilon}.
             In each case, we show the real parts of the pressure fields, and 
             the relative error with the reference 
             solution on a logarithmic scale. The imaginary part was also recovered but it is not shown.
             }} \label{OOD:set1}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%OOD2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{OOD 2}
We chose $3$ realizations of all the previously trained NNs, with the dataset at $15$ Hz, and the parameters  $\boldsymbol{\lambda} = (1, 1)$, wavespeed range of $[1500,5000]$, and we tested in another GRF. In this set family, we generate an anisotropic random field, different to the original trained data   ${\boldsymbol{\lambda}}_{\mathrm{OOD2}} = (0.10, 0.20)$, however the range was kept similar than the original set. The visualization of three random realizations of $c$ are presented in \cref{OOD:set2} for $15$Hz and only the real part of the field, the imaginary part is also recovered but not shown.

\begin{figure}[ht!]\centering
\input{Figures/OOD_main_paper/set1/skeleton_online_set1_appendix} 
    \caption{\small{ 
            %\textbf{(Real part) of the pressure field reconstructed by
             Pressure field reconstructed for 
             Experiment 2 (\cref{experiment2,figure:cp-GRF:experiment2}) 
             at frequency \num{15} \si{\Hz} trained with \emph{isotropic Whittle–Mat\'ern isotropic covariance} 
             $\boldsymbol{\lambda} = (1, 1)$, and wavespeed range of $(1500,5000)$ \cref{eq:lambda_cov} and from \cref{table:ood}
             ${\boldsymbol{\lambda}}_{\mathrm{OOD2}} = (0.10, 0.20)$, and wavespeed range of $(1500,5000)$
             with the different architectures for multiple realizations of the new GRF
             \emph{out-of distribution},
             realizations of the wave speed. 
             \textit{Left column} shows independent GRF realization of the wave
             speed (see \cref{Euler_equation}).  
             \textit{Second column} shows the real part % and imaginary part
             of the pressure field solution to the wave PDE at frequency
             15 \si{\Hz}, 
             obtained with software \texttt{hawen} \citep{faucher2021hawen}, 
             which we consider as the \emph{reference solution},
             see \cref{Euler_equation}. 
             \textit{Other columns} show the approximated reconstructions 
             using the different architectures:
             \textit{FNO}, see \citet{kovachki2021neural}; 
             $\multiplicative$ structure ($\MFNO$, see~\cref{MNO}); 
             and the solutions provided by $\FNONeXt$, \cref{FNO+epsilon}.
             In each case, we show the real parts of the pressure fields, and 
             the relative error with the reference 
             solution on a logarithmic scale. The imaginary part was also recovered but it is not shown.
             }}
             \label{OOD:set2}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%OOD3
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{OOD 3}
We chose $3$ realizations of all the previously trained NNs, with the dataset at $15$ Hz, and the parameters  $\boldsymbol{\lambda} = (1, 1)$, wavespeed range of $[1500,5000]$, and we tested in another GRF. In this set family, we generate an isotropic random field, different to the original trained data   ${\boldsymbol{\lambda}}_{\mathrm{OOD3}} = (0.20, 0.20)$, however the range was moved to $[2000,3500]$ different than the original set. The visualization of three random realizations of $c$ are presented in \cref{OOD:set3} for $15$Hz and only the real part of the field, the imaginary part is also recovered but not shown.



\begin{figure}[ht!]\centering
\input{Figures/OOD_main_paper/set2/skeleton_online_set2_appendix} 
    \caption{\small{ 
            %\textbf{(Real part) of the pressure field reconstructed by
             Pressure field reconstructed for 
             Experiment 2 (\cref{experiment2,figure:cp-GRF:experiment2}) 
             at frequency \num{15} \si{\Hz} trained with \emph{isotropic Whittle–Mat\'ern isotropic covariance} 
             $\boldsymbol{\lambda} = (1, 1)$, and wavespeed range of $(1500,5000)$ \cref{eq:lambda_cov} and from \cref{table:ood}
             ${\boldsymbol{\lambda}}_{\mathrm{OOD3}} = (0.20, 0.20)$, and wavespeed range of $(2000,3500)$
             with the different architectures for multiple realizations of the new GRF
             \emph{out-of distribution},
             realizations of the wave speed. 
             \textit{Left column} shows independent GRF realization of the wave
             speed (see \cref{Euler_equation}).  
             \textit{Second column} shows the real part % and imaginary part
             of the pressure field solution to the wave PDE at frequency
             15 \si{\Hz}, 
             obtained with software \texttt{hawen} \citep{faucher2021hawen}, 
             which we consider as the \emph{reference solution},
             see \cref{Euler_equation}. 
             \textit{Other columns} show the approximated reconstructions 
             using the different architectures:
             \textit{FNO}, see \citet{kovachki2021neural}; 
             $\multiplicative$ structure ($\MFNO$, see~\cref{MNO}); 
             and the solutions provided by $\FNONeXt$, \cref{FNO+epsilon}.
             In each case, we show the real parts of the pressure fields, and 
             the relative error with the reference 
             solution on a logarithmic scale. The imaginary part was also recovered but it is not shown.
             }}
             \label{OOD:set3}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%OOD4
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{OOD 4}
We chose $3$ realizations of all the previously trained NNs, with the dataset at $15$ Hz, and the parameters  $\boldsymbol{\lambda} = (1, 1)$, wavespeed range of $[1500,5000]$, and we tested in another GRF. In this set family, we generate an anisotropic random field, different to the original trained data   ${\boldsymbol{\lambda}}_{\mathrm{OOD4}} = (0.10, 0.20)$, however the range was kept to $[1500,5000]$ the same as the original set. The visualization of three random realizations of $c$ are presented in \cref{OOD:set4} for $15$Hz and only the real part of the field, the imaginary part is also recovered but not shown.


\begin{figure}[ht!]\centering
\input{Figures/OOD_main_paper/set3/skeleton_online_set3_appendix} 
    \caption{\small{ 
            %\textbf{(Real part) of the pressure field reconstructed by
             Pressure field reconstructed for 
             Experiment 2 (\cref{experiment2,figure:cp-GRF:experiment2}) 
             at frequency \num{15} \si{\Hz} trained with \emph{isotropic Whittle–Mat\'ern isotropic covariance} 
             $\boldsymbol{\lambda} = (1, 1)$, and wavespeed range of $(1500,5000)$ \cref{eq:lambda_cov} and from \cref{table:ood}
             ${\boldsymbol{\lambda}}_{\mathrm{OOD4}} = (0.10, 0.20)$, and wavespeed range of $(2000,3500)$
             with the different architectures for multiple realizations of the new GRF
             \emph{out-of distribution},
             realizations of the wave speed. 
             \textit{Left column} shows independent GRF realization of the wave
             speed (see \cref{Euler_equation}).  
             \textit{Second column} shows the real part % and imaginary part
             of the pressure field solution to the wave PDE at frequency
             15 \si{\Hz}, 
             obtained with software \texttt{hawen} \citep{faucher2021hawen}, 
             which we consider as the \emph{reference solution},
             see \cref{Euler_equation}. 
             \textit{Other columns} show the approximated reconstructions 
             using the different architectures:
             \textit{FNO}, see \citet{kovachki2021neural}; 
             $\multiplicative$ structure ($\MFNO$, see~\cref{MNO}); 
             and the solutions provided by $\FNONeXt$, \cref{FNO+epsilon}.
             In each case, we show the real parts of the pressure fields, and 
             the relative error with the reference 
             solution on a logarithmic scale. The imaginary part was also recovered but it is not shown.
             }}
             \label{OOD:set4}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%OOD5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{OOD 5}

We chose $3$ realizations of all the previously trained NNs, with the dataset at $15$ Hz, and the parameters  $\boldsymbol{\lambda} = (1, 1)$, wavespeed range of $[1500,5000]$, and we tested in another GRF. In this set family, we generate an isotropic random field, different to the original trained data   ${\boldsymbol{\lambda}}_{\mathrm{OOD5}} = (0.10, 0.30)$, however the range was also moved to $[2000,6000]$ different than the original set. The visualization of three random realizations of $c$ are presented in \cref{OOD:set5} for $15$Hz and only the real part of the field, the imaginary part is also recovered but not shown.


\begin{figure}[ht!]\centering
\input{Figures/OOD_main_paper/set4/skeleton_online_set4_appendix} 
    \caption{\small{ 
            %\textbf{(Real part) of the pressure field reconstructed by
             Pressure field reconstructed for 
             Experiment 2 (\cref{experiment2,figure:cp-GRF:experiment2}) 
             at frequency \num{15} \si{\Hz} trained with \emph{isotropic Whittle–Mat\'ern isotropic covariance} 
             $\boldsymbol{\lambda} = (1, 1)$, and wavespeed range of $(1500,5000)$ \cref{eq:lambda_cov} and from \cref{table:ood}
             ${\boldsymbol{\lambda}}_{\mathrm{OOD5}} = (0.10, 0.30)$, and wavespeed range of $(2000,6000)$
             with the different architectures for multiple realizations of the new GRF
             \emph{out-of distribution},
             realizations of the wave speed. 
             \textit{Left column} shows independent GRF realization of the wave
             speed (see \cref{Euler_equation}).  
             \textit{Second column} shows the real part % and imaginary part
             of the pressure field solution to the wave PDE at frequency
             15 \si{\Hz}, 
             obtained with software \texttt{hawen} \citep{faucher2021hawen}, 
             which we consider as the \emph{reference solution},
             see \cref{Euler_equation}. 
             \textit{Other columns} show the approximated reconstructions 
             using the different architectures:
             \textit{FNO}, see \citet{kovachki2021neural}; 
             $\multiplicative$ structure ($\MFNO$, see~\cref{MNO}); 
             and the solutions provided by $\FNONeXt$, \cref{FNO+epsilon}.
             In each case, we show the real parts of the pressure fields, and 
             the relative error with the reference 
             solution on a logarithmic scale. The imaginary part was also recovered but it is not shown.
             }}
             \label{OOD:set5}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%OOD6
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{OOD 6}\label{OOD:6}

We chose $3$ realizations of all the previously trained NNs, with the dataset at $15$ Hz, and the parameters  $\boldsymbol{\lambda} = (1, 1)$, wavespeed range of $[1500,5000]$, and we tested in another GRF. In this set family, we generate an anisotropic random field, \emph{significantly} different to the original trained data   ${\boldsymbol{\lambda}}_{\mathrm{OOD6}} = (0.25, 0.75)$, however the range was moved to $[2000,3500]$ different than the original set. The visualization of three random realizations of $c$ are presented in \cref{OOD:set6} for $15$Hz and only the real part of the field, the imaginary part is also recovered but not shown.

\begin{figure}[ht!]\centering
\input{Figures/OOD_main_paper/set5/skeleton_online_set5_appendix} 
    \caption{\small{ 
            %\textbf{(Real part) of the pressure field reconstructed by
             Pressure field reconstructed for 
             Experiment 2 (\cref{experiment2,figure:cp-GRF:experiment2}) 
             at frequency \num{15} \si{\Hz} trained with \emph{isotropic Whittle–Mat\'ern isotropic covariance} 
             $\boldsymbol{\lambda} = (1, 1)$, and wavespeed range of $(1500,5000)$ \cref{eq:lambda_cov} and from \cref{table:ood}
             ${\boldsymbol{\lambda}}_{\mathrm{OOD6}} = (0.25, 0.75)$, and wavespeed range of $(2000,6000)$
             with the different architectures for multiple realizations of the new GRF
             \emph{out-of distribution},
             realizations of the wave speed. 
             \textit{Left column} shows independent GRF realization of the wave
             speed (see \cref{Euler_equation}).  
             \textit{Second column} shows the real part % and imaginary part
             of the pressure field solution to the wave PDE at frequency
             15 \si{\Hz}, 
             obtained with software \texttt{hawen} \citep{faucher2021hawen}, 
             which we consider as the \emph{reference solution},
             see \cref{Euler_equation}. 
             \textit{Other columns} show the approximated reconstructions 
             using the different architectures:
             \textit{FNO}, see \citet{kovachki2021neural}; 
             $\multiplicative$ structure ($\MFNO$, see~\cref{MNO}); 
             and the solutions provided by $\FNONeXt$, \cref{FNO+epsilon}.
             In each case, we show the real parts of the pressure fields, and 
             the relative error with the reference 
             solution on a logarithmic scale. The imaginary part was also recovered but it is not shown.
             }}
             \label{OOD:set6}
\end{figure}
